Television Discourse Decoded: Comprehensive Multimodal Analytics at Scale

In this paper, we tackle the complex task of analyzing televised debates, with a focus on a prime time news debate show from India. Previous methods, which often relied solely on text, fall short in capturing the multimodal essence of these debates. To address this gap, we introduce a comprehensive automated toolkit that employs advanced computer vision and speech-to-text techniques for large-scale multimedia analysis. Utilizing state-of-the-art computer vision algorithms and speech-to-text methods, we transcribe, diarize, and analyze thousands of YouTube videos of a prime-time television debate show in India. These debates are a central part of Indian media but have been criticized for compromised journalistic integrity and excessive dramatization. Our toolkit provides concrete metrics to assess bias and incivility, capturing a comprehensive multimedia perspective that includes text, audio utterances, and video frames. Our findings reveal significant biases in topic selection and panelist representation, along with alarming levels of incivility. This work offers a scalable, automated approach for future research in multimedia analysis, with profound implications for the quality of public discourse and democratic debate. To catalyze further research in this area, we also release the code, dataset collected and supplemental pdf.

==> different_sections/ethics_checklist.tex <==
\section*{Ethics checklist}

\begin{enumerate}

\item For most authors...
\begin{enumerate}
    \item  Would answering this research question advance science without violating social contracts, such as violating privacy norms, perpetuating unfair profiling, exacerbating the socio-economic divide, or implying disrespect to societies or cultures?
    \answerYes{Yes}
  \item Do your main claims in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Yes}
   \item Do you clarify how the proposed methodological approach is appropriate for the claims made? 
    \answerYes{Yes}
   \item Do you clarify what are possible artifacts in the data used, given population-specific distributions?
    \answerYes{Yes.}
  \item Did you describe the limitations of your work?
    \answerYes{Yes.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Yes.}
      \item Did you discuss any potential misuse of your work?
    \answerYes{Yes.}
    \item Did you describe steps taken to prevent or mitigate potential negative outcomes of the research, such as data and model documentation, data anonymization, responsible release, access control, and the reproducibility of findings?
    \answerYes{Yes}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Yes}
\end{enumerate}

\item Additionally, if your study involves hypotheses testing...
\begin{enumerate}
  \item Did you clearly state the assumptions underlying all theoretical results?
    \answerNA{NA}
  \item Have you provided justifications for all theoretical results?
    \answerNA{NA}
  \item Did you discuss competing hypotheses or theories that might challenge or complement your theoretical results?
    \answerNA{NA}
  \item Have you considered alternative mechanisms or explanations that might account for the same outcomes observed in your study?
    \answerNA{NA}
  \item Did you address potential biases or limitations in your theoretical framework?
    \answerNA{NA}
  \item Have you related your theoretical results to the existing literature in social science?
    \answerNA{NA}
  \item Did you discuss the implications of your theoretical results for policy, practice, or further research in the social science domain?
    \answerNA{NA}
\end{enumerate}

\item Additionally, if you are including theoretical proofs...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{NA}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{NA}
\end{enumerate}

\item Additionally, if you ran machine learning experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{No}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Yes}
     \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Yes}
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{No}
     \item Do you justify how the proposed evaluation is sufficient and appropriate to the claims made? 
    \answerYes{Yes}
     \item Do you discuss what is ``the cost`` of misclassification and fault (in)tolerance?
    \answerYes{Yes}
  
\end{enumerate}

\item Additionally, if you are using existing assets (e.g., code, data, models) or curating/releasing new assets, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Yes}
  \item Did you mention the license of the assets?
    \answerNA{NA}
  \item Did you include any new assets in the supplemental material or as a URL?
    \answerNA{NA}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{Yes}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{Yes}
\item If you are curating or releasing new datasets, did you discuss how you intend to make your datasets FAIR (see \cite{fair})?
\answerYes{Yes}
\item If you are curating or releasing new datasets, did you create a Datasheet for the Dataset (see \cite{gebru2021datasheets})? 
\answerNA{NA}
\end{enumerate}

\item Additionally, if you used crowdsourcing or conducted research with human subjects, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots?
    \answerNo{No}
  \item Did you describe any potential participant risks, with mentions of Institutional Review Board (IRB) approvals?
    \answerYes{Yes}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNo{No}
   \item Did you discuss how data is stored, shared, and deidentified?
   \answerYes{Yes}
\end{enumerate}

\end{enumerate}
%\fi

==> prompts_used/get_labels.tex <==
\begin{table*}[h]
\caption{Prompt fed to LLAMA-2-13b-chat to fetch names from the transcriptGPT-3.5-Turbo to fetch the categories for the videos}
\label{tab:namescategory_fetch_prompt}
\begin{tabularx}{\linewidth}{|>{\raggedright\arraybackslash}X|}
\hline
Please map the below debate titles for debates conducted on an Indian news channel into different topics based on the title of the debates. One debate may belong to multiple topics. \\\\

\textbf{List of topics}:- [Politics, \sensitive{Supporting-BJP, Anti-BJP}, Anti-Opposition, State level politics, Scams, Religion, Economy, Defense \& Terrorism, International Affairs, COVID/Lockdown, Bollywood, Farmers Protest Issue, Ram Mandir Babri Masjid, Citizenship Amendment Act, Kashmir, Pakistan, Pulwama-Balakot, Crime and Justice, Sports, Education] \\

\textbf{Here is some additional context about topics:-} \\

- \sensitive{Supporting-BJP}: Debate titles that shows positive bias against BJP or BJP affiliated leaders. Eg: Why The Yogi Victory Is Historic 2022 Election Results. \\

- \sensitive{Anti-BJP}: Debate titles that shows negative bias against BJP or BJP affiliated leaders. Eg: Shouldn't UP CM Yogi Adityanath Rise Above Namecalling, Barbaric Cruelty' Allegation Against Seema Patra - BJP Suspends But No Arrest,Is Modi Wave On The Wane. \\

- Anti-Opposition: Debate titles that shows negative bias against Opposition such as Congress or criticisms about the Opposition affiliated leaders like Vadra and Gandhis. Eg: Will Priyanka Vadra Take Responsibility For Stampede At Children's Rally, PM Modi Sets Vision For 2047, Will Opposition Rise Above Petty Politics. \\

- Politics: Debates including day-to-day political developments with no broader themes and political debates with no clear bias in the title. Eg: Centre Launches 'Agnipath' For India - Is It A Gamechanger Or Not, Kharge Compares PM Modi To 'Ravan'. Will The Insult Politics Backfire \\

- State level politics: Debate titles with any mention of an Indian state or a state leader. Eg: Eknath Shinde Stakes Claim On Shiv Sena, Is MVA Govt's Time Up,Sanjay Raut Abuses Shinde Camp; Uddhav Thackeray Extends Olive Branch To Rebels, Tamil Nadu BJP Chief K Annamalai Speaks To Arnab, Threatens 'Mass Satyagraha' Over Fuel Price. \\\\

For each debate title and id, perform the following actions: \\
1 - Read the debate title \\
2 - Iterate through all topics in above list of topics and determine whether topic is relevant to the debate \\
3 - Keep track of all relevant topics to the debate. Note that some of the debates may be relevant to multiple topics. In such cases, include all the topics relevant. \\
Separate responses for separate debates with a newline. Provide them in JSON format with the following keys: \\
- debate\_id: \textless debate ID\textgreater, \\
- debate\_title: \textless debate title\textgreater, \\
- topics\_list: \textless list of topics mapped to\textgreater, \\
- reasoning: \textless Reasoning behind mapping\textgreater \\
\\
\textbf{Debate titles list (each debate on a new line with format: \textless debate ID\textgreater | \textless debate title\textgreater):} \\
AM4jNtwHX8k | Did Rahul Gandhi Link PM Modi To "Hindu Terror" \\
UK4WtrqwD1U | PM Modi Sold 'Chai' \& Not The Nation \\
a2GaKNHfLz0 | BIGGEST EXPOSE: Church Campaign Against Nationalism \\
lk-pPzP8K2g | Woman Misses Funeral Due To VVIP Racism \\
lbliEqB27nY | Rahul Gandhi To Lead The Congress Party \\
\hline
\end{tabularx}
\end{table*}


==> prompts_used/get_names.tex <==
\begin{table*}[h]
\caption{Prompt fed to LLAMA-2-13b-chat to fetch names from the transcript}
\label{tab:names_fetch_prompt}
\begin{tabularx}{\linewidth}{|>{\raggedright\arraybackslash}X|}
\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textless s\textgreater[INST] \textless\textless SYS\textgreater\textgreater\\You are a helpful, respectful and honest assistant. Always answer as helpfully as possible, while being safe.  Your answers should not include any harmful, unethical, racist, sexist, toxic, dangerous, or illegal content. Please ensure that your responses are socially unbiased and positive in nature.\\\\If a question does not make any sense, or is not factually coherent, explain why instead of answering something not correct. If you don't know the answer to a question, please don't share false information.\\\textless\textless SYS\textgreater\textgreater\\ \textit{Below within backticks is the transcript from a TV debate in India.    Extract the names of the speakers and panel members from the transcript.    HINT: the speakers are generally introduced in the beginning of the transcript by the debate moderator. Try using this introductory statement to find the names.     NOTE: Output the names as with numbering on new lines. In case the transcript has foul language, ignore the inappropriate language and personal attacks and focus only on finding the names.}    \\\\ \textbf{Transcript:} \\```\sensitive{Mumbai Studios of Republic TV. It's time for Arnab Goswami on the debate}. \\ \textbf{\textless speaker change\textgreater}\\  Good evening and welcome viewers. I don't believe in coincidences. The CBI director hates his number two and is fighting to stop him from taking over when he retires in a few weeks. The lawyer Prashant Bhushan steps in and challenges the appointment of the number two in the Supreme Court. 

This means that the CBI director obviously loves this and would love what Prashant Bhushan is doing for him. The CBI director then meets Prashant Bhushan and two people denied a birth in the Modi government. The permanently sulking Yashwant Sinha and Arun Shourie and Rafal. Viewers I'm asking you this, is this a coincidence? 

I may not name them viewers but now we all know who the lobby is. The lobby wants to engineer trouble within our country. Caste wars, they failed. Breaking down the Supreme Court, they failed. Dividing the Hindu religion, they failed. Destroying the agencies from within, they are trying. They will fail. It is our fundamental duty viewers, yours and mine, to make sure that they fail this time as well. We have to fight the lobby.

\textbf{\textless speaker change\textgreater}

....

\textbf{\textless speaker change\textgreater}
And if you will permit, Arnab this is basically, Arnab is, they tried it here, now they have hatched out to the CBI, hatched out to IP, for his role in the Godhra investigation, or his role, his question, his role in Gujarat came under huge question, his role in the Godhra investigation, his role in the Amit Shah case, so and then to bring him here, Mr. Modi lost the plot, he thinks, he thought he could run everything, but he can't, he has complete control of governance, of policy, they don't know the government can't do any policy, so please do not bring in this whole thing about casting us questions, if it's to our five investigative agents, in which we have been saying all the time, we are not even talking about policy, which they don't understand a word, but this is simple administrative issue.```
\\

[\slash INST]

\\\hline

\end{tabularx}

\end{table*}

==> tables_folder/negation.tex <==
\begin{table}
    \caption{Negation Words}
    \label{tab:negation_keywords}
    \begin{tabular}{|p{0.9\columnwidth}|}
        \hline
        not, don’t, can’t, won’t, shouldn’t, mustn’t, should not, must not, do not, cannot, will not, would not, wouldn’t, isn’t, is not, dare not, have not, might not, may not, need not, ought not, shall not \\
        \hline
    \end{tabular}
\end{table}

==> tables_folder/tag_category_mapping.tex <==
\begin{table*}[h]
\centering
\caption{Table showing \underline{some} categories and a \underline{subset} of their corresponding mapped tags}
\label{tab:tag_category_mapping}
\begin{tabular}{|p{0.2\linewidth}|p{0.8\linewidth}|}
\hline
\textbf{Category} & \textbf{Tags} \\ \hline
China & Tiktok banned | Xi Jinping | Sonia Gandhi Xi Jinping deal | modi xi jinping | xi jinping in india | XI jinping in Mamallapuram | Bharat vs China | Boycott China | india china international news | india china border news | China clashes | China Tawang border dispute | Chinese Apps TikTok blocked | LAC dispute \\ \hline
Triple Talaq & triple talaq debate | owaisi on triple talaq | triple talaq ordinance | arnab on triple talaq | triple talaq verdict | triple talaq banned \\ \hline
Ram Mandir Babri Masjid & babri masjid | ayodhya verdict | ram mandir ayodhya fight | subramanian swamy on ram mandir | tasleem rahmani on ayodhya | CBI Babri Masjid | ayodhya land settlement | Ayodhya case settlement | ram mandir 2025 | ayodhya march | cji impeachment linked to ayodhya | Ram MAdir politics | Ayodha mediation panel \\ \hline
Sports & t20 world cup | icc t20 world cup 2022 | IPL | india backs ms dhoni | ms dhoni | indian football | indian football team | fifa banned india | RCB | MI | Virat Kohli Captaincy | arbaaz khan ipl betting case | ipl betting scandal \\ \hline
Covid & China virus | Covishield | Vaccine in India | covishield | rahul gandhi questions vaccine | Is Covishield safe | Vaccine registration | 21 day lockdown | lockdown extension | coronavirus disease | covid china | covid origin | corona in india social media | pm modi on covid vaccine | lockdown violators | Coronavirus India lockdown | lockdown 21 day | 21 days lockdown | Modi coronavirus lockdown | Coronavirus warriors attacked \\ \hline
Pulawama Balakot & major gaurav arya on pulwama | pulwama terror attack | surgical strike | gen gd bakshi on surgical strike | Pulwama attack | avenge pulwama | pm modi on surgical strike | Surgical Strike \\ \hline
Farmers Protest & farmer protest | Farmer Bill 2020 | govt farmer talks | Centre Farmer talks | Farm Bill 2020 | Farm Bills explained | Three Farm Bills | sc hearing on farm law | haryana farmers protest live | haryana farmers protest latest | haryana farmers protest study iq | haryana farmers protest lallantop \\ \hline
Bollywood & Deepika Padukone | Sara Ali Khan | bollywood drug party | kangana ranaut interview | ncb summons bollywood | Aryan Khan drugs case | richa chadha on indian army | me too campaign \\ \hline
Republic TRP Scam Case and Other Republic Related & FIR against Republic TV | Param Bir Singh case | fake trp | Param Bir Sachin Vaze secret meet | Sadhvi Pragya exposes Param Bir Singh | cbi fir trp scam case | arnab goswami trp scam | trp scam cbi | Param Bir Extortion racket | Republic Editorial Staff FIR \\ \hline
Economy & budget 2019 | nirmala sitharaman budget | union budget 2022 highlights | PM modi Economy push | rahul gandhi on fuel price | demonetization india | pm modi on fuel prices | arun jaitley gst | Make in India \\ \hline
Regional Elections & tamil nadu election | tamil nadu election 2021 | tamil nadu politics | tamil nadu assembly election 2021 | Tamil Nadu 2021 2021 elections | gujarat elections | UP elections | Uttar Pradesh Polls | UP polls 2022 \\ \hline
2019 Elections & elections 2019 | 2019 lok sabha elections | who will win 2019 | election opinion poll 2019 | modi back in 2019 | modi sweep back in 2019 | manifesto 2019 | rahul gandhi 2019 manifesto | 2019 election survey | third front 2019 | bjp vs congress 2019 \\ \hline
Sabarimala Case & Politics on Sabarimala | sabarimala updates | sabarimala temple issue | womens entry in sabarimala | sabarimala verdict supreme court | trupti desai on sabarimala | rahul easwar sabarimala debate | sabarimala protest pandalam \\ \hline
\end{tabular}
\end{table*}

==> tables_folder/tags_example.tex <==
\begin{table}
\centering
\captionsetup{width=\linewidth}
\caption{Few examples of tags associated with the various videos}
\label{tab:tags_example}
\begin{tabularx}{\linewidth}{|>{\hsize=0.3\hsize}X|>{\hsize=0.7\hsize}X|}
\hline
\textbf{Title} & \textbf{Tags} \\
\hline
\href{https://www.youtube.com/watch?v=ec9X8bC96Eo}{CBI To Probe 'Witness Coercion' Tapes, Param Bir In Deep Trouble} & CBI TRP case, Witness tapes, TRP case manipulation, TRP witness scam, TRP witness coercion tapes, india today trp scam, republic tv fake trp, india today fake trp \\
\hline
\href{https://www.youtube.com/watch?v=Mdj3BrofgUI}{Justice For Sushant: Demand Grows For CBI Investigation} & Sushant Singh rajput, Sushant Singh Rajput soul talks, Sushant Singh Rajput murdered by Suraj Pancholi, Rumi Jaffery, Mumbai Police Sushant Singh,Sushant Singh Rajput spirit calling, Kangana Ranaut, Kangana Ranaut Sushant Singh, Kangana Ranaut \\
\hline
\href{https://www.youtube.com/watch?v=PRrQCwnrH0Y}{Jyotiraditya Scindia's Exit Stings Congress} & Sonia Gandhi, Rahul Gandhi, maharashtra politics, maharashtra government, maha vikas aghadi rift, NCP, Shiv sena, uddhav thackeray, sharad Pawar, Priyanka Gandhi, Scinida, jyotiraditya scindia, jyotiraditya scindia bjp join,  jyotiraditya scindia quits congress \\
\hline
\href{https://www.youtube.com/watch?v=-jU1IBxhGrU}{Nation backs MS Dhoni Wearing The `Balidaan Badge'} & indian premier league, Balidaan Badge, balidaan badge controversy, glove controversy, india backs ms dhoni, national pride, balidan badge indian army, ms dhoni, world cup 2019 indian team, bcci, indian cricket team, 2019 world cup indian team, bcci writes to ICC \\
\hline
\href{https://www.youtube.com/watch?v=Oy3aJ18FMoY}{Will Yogi Adityanath Sack Rape Accused MLA?} & cm yogi adityanath, unnao rape case, kuldeep singh sengar, bjp mla rape case, mla rape case, rape victim father death, cbi investigation of unnao, uttar pradesh, unnao case, bjp mla brother arrested, up police on unnao, cm yogi on unnao case \\
\hline
\end{tabularx}
\end{table}

==> tables_folder/triads_incivility_table.tex <==
\begin{table}[h]
    \centering
     \caption{Affiliation Triads with a statistically significant difference in incivility compared to overall incivility. Incivility values here are the sum of overlap and toxicity.}
    \label{tab:triad_incivility}
    \begin{tabular}{|p{0.3\columnwidth}|p{0.3\columnwidth}|p{0.3\columnwidth}|}
    \hline
    Triad & Average incivility fraction in videos where they occur & Frequency of them occurring in a video \\ 
    \hline
    DMK-BJP-BJP & 0.218 & 72 \\
    \hline
    Congress-BJP-AAP & 0.209 & 52 \\
    \hline
    BJP-AAP-BJP & 0.204 & 88 \\
    \hline
    BJP-Samajwadi party-BJP & 0.189 & 70 \\
    \hline
    TMC-BJP-BJP & 0.179 & 148 \\
    
    \hline
    \end{tabular}
\end{table}

